A Categorical Approach to Subgroups of Quantum Groups and Their Crystal Bases

Suppose that we have a semisimple, connected, simply connected algebraic group $G$ with corresponding Lie algebra $\mathfrak{g}$. There is a Hopf pairing between the universal enveloping algebra $U(\mathfrak{g})$ and the coordinate ring $O(G)$. By introducing a parameter $q$, we can consider quantum deformations $U_q(\mathfrak{g})$ and $O_q(G)$ respectively, between which there again exists a Hopf pairing. We show that the category of crystals associated with $U_q(\mathfrak{g})$ is a monoidal category. We define subgroups of $U_q(\mathfrak{g})$ to be right coideal subalgebras, and subgroups of $O_q(G)$ to be quotient left $O_q(G)$-module coalgebras. Furthermore, we discuss a categorical approach to subgroups of quantum groups which we hope will provide us with a link to crystal basis theory.

==> diagrams/hopf.tex <==

\begin{tikzcd}[row sep=3.6em,column sep=1em]
& H\otimes H \arrow[rr,"S\otimes \text{id}_H"] && H\otimes H \arrow[dr,"\mu"] \\
H \arrow[ur,"\Delta"] \arrow[rr,"\varepsilon"] \arrow[dr,"\Delta"'] && k \arrow[rr,"\eta"] && H \\
& H\otimes H \arrow[rr,"\text{id}_H\otimes S"'] && H\otimes H \arrow[ur,"\mu"']
\end{tikzcd}

==> diagrams/onetoone.tex <==
\begin{tikzpicture}

\node(a) at (0,0) {right coideal subalgebras of $H$};
\node(b) at (8,0) {quotient left module coalgebras of $H$};
\node(c) at (4,1.7) {$A\rightarrow{H/HA^+}$};
\node(d) at (4,-1.7){${}^C H\leftarrow{C}$};
\draw [->] (a) to [out=30,in=150] (b);
\draw [->] (b) to [out=-150,in=-30] (a);
\end{tikzpicture}

==> diagrams/triangle3.tex <==
$\begin{tikzcd}
I\otimes A \arrow[r, "e\otimes 1_A"] \arrow[dr,"l_A"]
& A\otimes A \arrow[d, "m"] 
& A\otimes I \arrow [l,"1_A\otimes e" above] \arrow[dl, "r_A" above]\\
& A
\end{tikzcd}$



